The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning

We consider the problem of training a $d$ dimensional model with distributed differential privacy (DP) where secure aggregation (SecAgg) is used to ensure that the server only sees the noisy sum of $n$ model updates in every training round. Taking into account the constraints imposed by SecAgg, we characterize the fundamental communication cost required to obtain the best accuracy achievable under $\varepsilon$ central DP (i.e. under a fully trusted server and no communication constraints). Our results show that $\tilde{O}\left( \min(n^2\varepsilon^2, d) \right)$ bits per client are both sufficient and necessary, and this fundamental limit can be achieved by a linear scheme based on sparse random projections. This provides a significant improvement relative to state-of-the-art SecAgg distributed DP schemes which use $\tilde{O}(d\log(d/\varepsilon^2))$ bits per client. Empirically, we evaluate our proposed scheme on real-world federated learning tasks. We find that our theoretical analysis is well matched in practice. In particular, we show that we can reduce the communication cost significantly to under $1.2$ bits per parameter in realistic privacy settings without decreasing test-time performance. Our work hence theoretically and empirically specifies the fundamental price of using SecAgg.

==> The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning (arxiv)_arXiv/content/1introduction.tex <==
Federated learning (FL) is a widely used machine learning framework where multiple clients collaborate in learning a model under the coordination of a central server~\citep{mcmahan2017communication,aopfl}. 
One of the primary attractions of FL is that it provides data confidentiality and can provide a level of privacy to participating clients through data minimization: the raw client data never leaves the device, and only updates to models (e.g., gradient updates) are sent back to the central server. 
This provides practical privacy improvements over centralized settings because updates typically contain less information about the clients, because they are more focused on the learning task, and also only need to be held ephemerally by the server


However, this vanilla federated learning does not provide any formal or provable privacy guarantees.
To do so, FL is often combined with  differential privacy (DP)~\citep{dwork2006calibrating}. 
This can be done in one of two ways\footnote{Local DP is yet another alternative, but it incurs higher utility loss and is therefore not typically used in practice.}: 1) perturbing the aggregated (local) model updates at the server before updating the global model, or 2) perturbing each client's model update locally and using a cryptographic multi-party computation protocol to ensure that the server only sees the noisy aggregate.
The former is referred to as \emph{central} DP, and it relies on the clients' trust in the server because any sensitive information contained in the model updates is revealed to and temporally stored on the server. The latter is referred to as \emph{distributed} DP \citep{dwork2006our, kairouz2021distributed, agarwal2021skellam, agarwal2018cpsgd}, and it offers privacy guarantees with respect to an \emph{honest-but-curious} server. Thus, a key technology for formalizing and strengthening FL’s privacy guarantees is a secure vector sum protocol called secure aggregation (SecAgg)~\citep{bonawitz2016practical, bell2020secure}, which lets the server see the aggregate client updates but not the individual ones.

Despite enhancing the clients' privacy, aggregating model updates via SecAgg drastically increases the computation and communication overheads~\citep{bonawitz2016practical, bonawitz2019towards}. This is even worse in federated settings where communication occurs over bandwidth-limited wireless links, and the extra communication costs may become a bottleneck that hampers efficient training of large-scale machine learning models. For example,~\citet{kairouz2021distributed} reports that when training a language model with SecAgg and DP, even with a carefully designed quantization scheme, each client still needs to transmit about $16$ bits \emph{per model parameter} each round. Moreover, the bitwidth needs to be scaled up when the privacy requirements are more stringent. This behavior disobeys the conclusion of~\citet{chen2020breaking} (derived under local DP), which shows that the optimal communication cost should \emph{decay} with the privacy budget, i.e., data is more compressible in the high privacy regime.

Furthermore, because the server aggregates the model updates via SecAgg, we can only compress the model updates locally using linear schemes. This constraint rules out many popular compression schemes such as entropy encoders or gradient sparsification \citep{aji2017sparse, lin2017deep, wangni2017gradient, havasi2018minimal, oktay2019scalable} etc., as these methods are non-linear. 

Therefore, it is unclear whether or not the communication cost of SecAgg reported in~\citet{kairouz2021distributed, agarwal2021skellam, agarwal2018cpsgd} is fundamental. If not, what is the smallest communication needed to achieve distributed DP with secure aggregation to achieve the same performance as in the centralized DP setting?

In this paper, we answer the above question, showing that the communication costs of existing mechanisms are strictly sub-optimal in the distributed mean estimation (DME) task \citep{an2016distributed} (see Section~\ref{sec:formulation} for details). We also propose a SecAgg comaptible \emph{linear} compression scheme based on sparse random projections (Algorithm~\ref{alg:sketch_mean_decoder}), and then combine it with the distributed discrete Gaussian (DDG) mechanism proposed by~\citet{kairouz2021distributed}. Theoretically, we prove that our scheme requires $\tilde{O}\lp \min(n^2\varepsilon^2, d) \rp$ bits per client, where $n$ is the per-round number of clients. This cost is significantly smaller than the communication cost of previous schemes which was $\tilde{O}_\delta(d\log(d/\varepsilon^2))$ bits per client\footnote{For simplicity, we use the $\tilde{O}_\delta\lp \cdot\rp$ notation to hide the dependency on $\delta$ and $\log n$}. To give perspective, 
(1) $n$ is usually on the order of $10^3$ per round due to the computational overhead of SecAgg, and (2) $\varepsilon$ is the privacy budget for a single round, i.e., $\varepsilon \approx {\varepsilon_{\msf{final}}}/{\sqrt{R}}$ if there are $R$ training rounds. Thus, for practical FL settings where large models are trained with SecAgg over many rounds, $n^2\varepsilon^2$ is typically (much) smaller than $d$. 

We complement our achievability results with a matching lower bound, showing that to obtain an unbiased estimator of the mean vector, each client needs to communicate $\tilde{\Omega}(\min(n^2\varepsilon^2, d))$ bits with the server. Our upper and lower bounds together specify the fundamental privacy-communication-accuracy trade-offs under SecAgg and DP.


In addition, we show that with additional sparsity assumptions, we can further improve both the accuracy and communication efficiency while achieving the same privacy requirement, leading to a logarithmic dependency on $d$.

Empirically, we verify our scheme on a variety of real-world FL tasks. Compared to existing distributed DP schemes, we observe $10$x or more compression with no significant decrease in test-time performance. Moreover, the compression rates can be made even higher with tighter privacy constraints (i.e., with smaller $\varepsilon$), complying with our theoretical $\tilde{O}(\min(n^2\varepsilon^2, d)$ communication bound.  


\paragraph{Organization}
The rest of this paper is organized as follows. We summarize related work in Section~\ref{sec:related} and introduce necessary preliminaries in Section~\ref{sec:preliminary}. We then provide a formal problem formulation in Section~\ref{sec:formulation}. Next, we present and analyze the performance of our main scheme (in terms of privacy, utility, and communication efficiency) and prove its optimality in Section~\ref{sec:worstcase}. After that, we show, in Section~\ref{sec:sparse}, that with additional sparsity assumptions, one can simultaneously reduce the communication cost and increase the accuracy. Finally, we present our experimental results in Section~\ref{sec:experiments} and conclude the paper in Section~\ref{sec:conc}.



==> The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning (arxiv)_arXiv/content/2related_works.tex <==
\paragraph{SecAgg and distributed DP}
SecAgg is cryptographic secure multi-party computation (MPC) that allows the server to collect the sum of $n$ vectors from clients without knowing anyone of them. In our single-server FL setting, SecAgg is achieved via additive masking over a finite group \citep{bonawitz2016practical, bell2020secure}. However, the vanilla FL with SecAgg does not provide provable privacy guarantees since the sum of updates may still leak sensitive information \citep{melis2019exploiting, song2019auditing, carlini2019secret, shokri2017membership}. To address this issue, differential privacy (DP) \citep{dwork2006our}, and in particular, DP-SGD or DP-FedAvg can be employed \cite{song2013stochastic, bassily2014private, geyer2017differentially, mcmahan2017learning}. In this work, we aim to provide privacy guarantees in the form of R\'enyi DP \citep{mironov2017renyi} because it allows for accounting end-to-end privacy loss tightly.

We also distinguish our setup from the local DP setting \citep{kasiviswanathan2011can, evfimievski2004privacy, warner1965randomized}, where the data is perturbed on the client-side before it is collected by the server. Local DP, which allows for a possibly malicious server, is stronger than distributed DP, which assumes an honest-but-curious server. Thus, local DP suffers from worse privacy-utility tarde-offs~\citep{kasiviswanathan2011can,duchi2013local, kairouz16}.


\paragraph{Model compression, sketching, and random projection}
There has been a significant amount of recent work on reducing the communication cost in FL, see \citet{kairouz2019advances}. Among them, popular compression approaches include gradient quantization \citep{alistarh17qsgd, bernstein2018signsgd}, sparsification \citep{aji2017sparse, lin2017deep, wangni2017gradient}, and entropy encoders \citep{havasi2018minimal, oktay2019scalable}. However, since these schemes are mostly non-linear, they cannot be combined with SecAgg where all the encoded messages will be summed together. Therefore, in this work, we resort to compression schemes with \emph{linear} encoders. The only exception are sketching based methods \citep{rothchild2020fetchsgd, haddadpour2020fedsketch}. Our work differs from them in three aspects. First, we consider FL with privacy and SecAgg, whereas \cite{rothchild2020fetchsgd} only aims at reducing communication. Second, although we use the same count-sketch encoder, our decoding method is more aligned with the sparse random projection \citep{kane2014sparser}. In the language of sketching, we decode the sketched model updates by ``count-mean'' instead of count-median, which improves space efficiency, thus requiring less memory to train a real-world large-scale machine learning model. We note that both count-sketch and random projection provides the same worst-case $\ell_2$ error bounds. 

\paragraph{FL with SecAgg and distributed DP}
The closest works to ours are cpSGD~\citep{agarwal2018cpsgd}, DDG~\citep{kairouz2021distributed}, and Skellam~\citep{agarwal2021skellam}, which serve as the main inspiration of this paper. However, all of these methods rely on per parameter quantization and thus lead to $\tilde{\Omega}\lp d \rp$ communication cost. In this work, however, we show that when $d \gg n^2\varepsilon^2$,  we can further reduce dimensionality and achieve the optimal communication cost  $\tilde{O}(n^2\varepsilon^2)$ in this regime. Our scheme also demonstrates $10$x or more compression rates (depending on the privacy budget) relative to the best existing distributed DP schemes. 

==> The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning (arxiv)_arXiv/content/3preliminary.tex <==
\subsection{Differential Privacy}
We begin by providing a formal definition for $(\varepsilon, \delta)$-differential privacy (DP) \cite{dwork2006calibrating}.
\begin{definition}[Differential Privacy]\label{def:DP}
For $\varepsilon, \delta \geq 0$, a randomized mechanism $M$ satisfies $(\varepsilon, \delta)$-DP if for all neighboring datasets $D, D'$ and all $\mcal{S}$ in the range of $M$, we have that 
$$ \Pr\lp M(D) \in \mcal{S} \rp \leq e^\varepsilon \Pr\lp M(D') \in \mcal{S} \rp+\delta,  $$
where $D$ and $D'$ are neighboring pairs if they can be obtained from each other by adding or removing all the records that belong to a particular user.
\end{definition}
The above DP notion is referred to as user level DP and is stronger than the commonly-used item level DP, where, if a user contributes multiple records, only the addition or removal of one record is protected.


We also make use of Renyi differential privacy (RDP) which allows for tight privacy accounting.
\begin{definition}[Renyi Differential Privacy]\label{def:RDP}
A randomized mechanism $M$ satisfies $(\alpha, \varepsilon)$-RDP if for any two neighboring datasets $D, D'$, we have that $D_\alpha\lp P_{M(D)}, P_{M(D')} \rp\leq \varepsilon$ where $D_{\alpha}\lp P, Q\rp$ is the Renyi divergence between $P$ and $Q$ and is given by 
$$ D_\alpha\lp P, Q \rp \eqDef \frac{1}{\alpha}\log\lp \E_{Q}\lb \lp \frac{P(X)}{Q(X)} \rp^\alpha \rb \rp.$$
\end{definition}
Notice that one can convert $(\alpha, \varepsilon(\alpha))$-RDP to $(\varepsilon_\msf{DP}(\delta), \delta)$-DP using the following lemma from \citet{asoodeh2020better, canonne2020discrete, bun2016concentrated}:
\begin{lemma}\label{lemma:rdp_to_approx_dp}
    If $M$ satisfies $\lp \alpha, \varepsilon \rp$-RDP, then, for any $\delta > 0$, $M$ satisfies $\lp \varepsilon_{\msf{DP}}(\delta), \delta \rp$, where
$$ \varepsilon_{\msf{DP}}(\delta) = \varepsilon+\frac{\log\lp 1/\alpha\delta \rp}{\alpha-1}+\log(1-1/\alpha). $$
\end{lemma}


\subsection{The Distributed Discrete Gaussian Mechanism}\label{sec:ddg}
The previous work of \citet{kairouz2021distributed} proposed a scheme based on the discrete Gaussian mechanism (denoted as $\texttt{DDG}$) which achieves the best mean square error (MSE) $O\lp \frac{c^2d}{n^2\varepsilon^2} \rp$ with a $\frac{1}{2}\varepsilon^2$-concentrated differential privacy guarantee. The encoding scheme mainly consists of the following four steps: (a) scaling, (b) random rotation (therein flattening), (c) conditional randomized rounding, and (d) perturbation, which we summarize in Algorithm~\ref{alg:ddg_simplified} below.




\begin{algorithm}[tbh]
\caption{The DDG mechanism}\label{alg:ddg_simplified}
    \begin{algorithmic}
	\STATE \textbf{Inputs:} Private vector $x_i\in \mbb{R}^d$; clipping threshold $c$;  modulus $M \in \mbb{N}$; noise scale $\sigma > 0$;
	
	\STATE Clip and scale $x_i$ so that $\lV x'_i \rV_2 < c$\;%
	\STATE Randomly rotate vector: $x''_i = U_{\msf{rotate}}\cdot x_i'$%
	\STATE Stochastically round and discretize $x_i''$ into $x_i''' \in \mbb{Z}^d$
	\STATE $Z_i = x'''_i + \mcal{N}_{\mbb{Z}}(0, \sigma^2) \mod{M}$, where $\mcal{N}_{\mbb{Z}}$ is the discrete Gaussian noise\;
	\STATE\textbf{Return:} $Z_i \in \mbb{Z}_M^d$
	\end{algorithmic}
\end{algorithm}


Upon aggregating $\hat{\mu}_{z} = \sum_{i\in[n]} Z_i$, the server can rotate $\hat{\mu}_z$ reversely and re-scale it back to decode the mean $\hat{\mu} =\frac{1}{n}\sum_i x_i$. We refer the reader to Algorithm~\ref{alg:ddg_detailed} in the appendix for a detailed version of DDG. By picking the parameters properly (see Theorem~\ref{thm:ddg}), Algorithm~\ref{alg:ddg_simplified} has the following properties:
\begin{itemize}
\setlength\itemsep{0.1em}
    \item Satisfies $(\alpha, \frac{\varepsilon^2}{2}\alpha)$-RDP, which implies $(\varepsilon_\msf{DP}, \delta)$-DP  with $\varepsilon_\msf{DP} = O_{\delta}\lp \varepsilon^2 \rp$%
    \item Uses  $O\lp d\log\lp n+\sqrt{\frac{n^3\varepsilon^2}{d}}+\frac{\sqrt{d}}{\varepsilon}\rp\rp$ bits of per client
    \item Has an MSE of $ \E\lb \lV \hat{\mu} - \mu \rV^2_2 \rb= O\lp \frac{c^2d}{n^2\varepsilon^2} \rp$.
\end{itemize}



\subsection{Sparse random projection and count-sketch}\label{sec:sparse_random_projection}
We now provide background on sparse random projection~\cite{kane2014sparser} and count-sketching, which allows us to reduce the dimension of local gradients from $\mbb{R}^d$ to $\mbb{R}^m$ with $m \ll d$. These schemes are \emph{linear}, making them compatible with \SA. 


Let $S_1,...,S_t \in \lbp -1, 0, 1 \rbp^{d\times w}$ be $t$ identical and independent count-sketch matrices, that is, \begin{equation}\label{eq:S}
    \lp S_i\rp_{j, k} = \sigma_i(j)\cdot\bbm{1}_{\lbp h_i(j)=k\rbp},
\end{equation}
for some independent hash functions $h_i:[d] \ra [w]$ and $\sigma_i:[d]\ra\lbp -1, +1\rbp$. Let $m = t\times w$, then the sparse random projection matrix $S\in \mbb{R}^{d \times m}$ is then defined as stacking $S_1,...,S_t$ vertically, that is,
\begin{equation}\label{eq:def_S}
    S^\intercal = \frac{1}{\sqrt{t}}
\begin{bmatrix}
S^\intercal_1, S^\intercal_2,...,S_t^\intercal
\end{bmatrix}.
\end{equation}

Under this construction, $S$ is sparse in the sense that each column contains exactly $t$ $1$s. We introduce several several nice properties that $S$ possesses which will be used in our analysis.

The following two lemmas controls the distortion of the embedded vector $S\cdot g$ for a $g \in \mbb{R}^d$.
\begin{lemma}\label{lemma:proj_var_bdd}
Let $S$ be defined as in \eqref{eq:def_S}. For any $g_1, g_2 \in \mbb{R}^d$, $\E\lb g_1^\intercal S^\intercal S g_2 \rb = \lan g_1, g_2 \ran$ and
\begin{align*}
    \E_{S}\lb \lan Sg_1, Sg_2\ran^2 \rb \leq \lan g_1, g_2\ran^2 + \frac{2}{m}\lV g_1\rV_2^2\cdot\lV g_2\rV_2^2.
\end{align*}
Furthermore, for any $g \in \mcal{R}^d$,
\begin{align}\label{eq:proj_var_bdd}
    \E_S\lb\lV S^\intercal Sg-g\rV^2_2\rb \leq \frac{2d}{m}\lV g \rV^2_2.
\end{align}
\end{lemma}
The proof follows by directly computing $\E_{S}\lb \lan Sg_1, Sg_2\ran^2 \rb$ (which can be written as a quadratic function of $S$ and $g_1$, $g_2$). See, for instance, Lemma~D.15 in \cite{anonymous2022iterative}.

\begin{lemma}[Sparse Johnson-Lindenstrauss lemma \citep{kane2014sparser}]\label{lemma:SJL}
Let $S$ be defined in \eqref{eq:def_S} and let $g \in \mbb{R}^d$. Then as long as $m \geq \Theta\lp \frac{1}{\alpha^2}\log\lp \frac{1}{\beta} \rp \rp$ and $t \geq \Theta\lp \frac{1}{\alpha} \log\lp \frac{1}{\beta} \rp \rp$, 
\begin{align}
    \Pr\lbp \lV S\cdot g \rV^2_2 \geq (1+\alpha)\lV g\rV^2_2 \rbp \leq \beta.
\end{align}
\end{lemma}

Finally, Lemma~\ref{lemma:inverse_sketch} states that the ``unsketch'' operator preserves the $\ell_2$ norm.
\begin{lemma}\label{lemma:inverse_sketch}
    Let $S, m, t$ be defined in \eqref{eq:def_S} and $v \in \mbb{R}^m$ (which can possibly depends on $S$) with $\E\lb\lV v \rV^2_2| S\rb \leq B^2$ almost surely. Then 
    it holds that $ \E\lb \lV S^\intercal v \rV^2_2\rb \leq \frac{8dB^2}{m}. $
\end{lemma}


==> The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning (arxiv)_arXiv/content/4formulation.tex <==

We start by formally presenting the distributed mean estimation (DME) \cite{an2016distributed} problem under differential privacy. Note that DME is closely related to the federated averaging (FedAvg) algorithm \cite{mcmahan2017communication}, where in each round, the server updates the global model using a noisy estimate of the mean of local model updates. Such a noisy estimate is typically obtained via a DME mechanism, and thus one can easily build a DP-FedAvg scheme from a DP-DME scheme.

\paragraph{Distributed mean estimation under differential privacy}
Consider $n$ clients each with a data vector $x_i \in \mathbb{R}^d$ that satisfies $\lV x_i \rV_2 \leq c$ 
(e.g., a clipped local model update). After communicating with $n$ clients, a server releases a noisy estimates $\hat{\mu}$ of the mean $\mu \triangleq \frac{1}{n}\sum_i x_i$, such that 1) $\hat{\mu}$ satisfies a differential privacy constraint (see Definition~\ref{def:DP} and Definition~\ref{def:RDP}), and 2) $\E\lb \lV \hat{\mu} - \mu \rV^2_2 \rb$ is minimized. The goal is to design a communication protocol (which includes local encoders and a central decoder) and an estimator $\hat{\mu}$.

In this paper, we consider two different DP settings. The first is the \textit{centralized}  DP setting: the server has access to all $x_i$'s, i.e., $\hat{\mu} = \hat{\mu}\lp x_1,...,x_n \rp$.
The  second is the \textit{distributed} DP via \SA setting: under this setting, each client is subject to a $b$-bit communication constraint, so they must first encode $x_i$ into a $b$-bit message, i.e., $Z_i = \mcal{A}_{\msf{enc}}(x_i) \in \mcal{Z}$ with $\lba\mcal{Z}\rba \leq 2^b$ (See Figure~\ref{fig1} for an illustration). However, instead of directly collecting $Z_1,...,Z_n$, the server can only observe the \emph{sum} of them, so the estimator must be a function of $\sum_{i=1}^n Z_i$ (i.e., $\hat{\mu} = \hat{\mu}\lp \sum_{i=1}^n Z_i \rp$). Moreover, we require that the sum $\sum_i Z_i$ satisfies DP (which is stronger than requiring $\hat{\mu}$ to be DP), meaning that individual information will not be disclosed to the server as well. Notice that since \SA operates on a finite additive group, we require $\mcal{Z}$ to have an additive structure. Without loss of generality, we will set $\mcal{Z}$ to be $\lp\mbb{Z}_M\rp^m$ for some $m, M \in \mbb{N}$, where $\mbb{Z}_M$ denotes the group of integers modulo $M$ (equipped with modulo $M$ addition) and $m$ is the dimension of the space we are projecting onto. In other words, we allocate $\log M$ bits for every coordinate of the projected vector. Note that in this case, the total per-client communication cost is $b = m\log M$.%

\begin{figure}[ht]
\begin{center}
{\includegraphics[width=0.5\linewidth]{./figures/secAgg.png}}
\caption{Private mean estimation via SecAgg.}
\label{fig1}
\end{center}
\end{figure} 

For a fixed privacy constraint, the fundamental problem we seek to solve is: what is the smallest communication cost under the distributed DP setting needed to achieve the accuracy of the centralized DP setting? Further, we seek to discover schemes that (a) achieve the optimal privacy-accuracy-communication trade-offs and (b) are memory efficient and computationally fast in encoding and decoding.

==> The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning (arxiv)_arXiv/content/5worstcase.tex <==

In this section, we characterize the \emph{optimal communication cost} under the distributed DP via SecAgg setting, defined as the smallest number of bits (as a function of $n, d, \varepsilon$) needed to achieve the same accuracy (up to a constant factor) of the centralized setting under the same $(\varepsilon, \delta)$-DP constraint. 


\paragraph{Optimal MSE under central DP} 

We start by specifying the optimal accuracy under a fully trusted server and no communication constraints. Under a DME setting where $\lV x_i \rV_2 \leq c$ for all $i\in[n]$, the $\ell_2$ sensitivity of the mean query $\mu(x_1,...,x_n) \eqDef \frac{1}{n}\sum_{i=1}^n x_i$ is bounded by 
$$ \Delta\lp \mu \rp \eqDef \max_{x^n, x_1'} \lV \mu(x_1,...,x_n) - \mu(x_1',...,x_n) \rV_2^2 \leq \frac{2c^2}{n}.  $$
Therefore, to achieve ($\varepsilon, \delta)$ central DP, the server can add coordinate-wise independent Gaussian noise to $\mu$. This gives an $\ell_2$ error that scales as 
$O_{\delta}\lp \frac{c^2d}{n^2\varepsilon^2} \rp$, which is known to be tight in the high privacy regime \cite{kamath2020primer}. Moreover, the resulting estimator is \emph{unbiased}\footnote{Notice that in this work, we are mostly interest in unbiased estimators (see Remark~\ref{rmk:unbiasedness} for a discussion).}.



\paragraph{Communication costs of DDG}
Next, we examine the communication costs of previous distributed DP schemes such as the DDG mechanism. As mentioned in Section~\ref{sec:ddg} and Theorem~\ref{thm:ddg}, in order to achieve the $O_{\delta}\lp \frac{c^2d}{n^2\varepsilon^2} \rp$ error, the communication cost of DDG must to be at least $\Theta\lp d \log\lp d/\varepsilon^2 \rp \rp$ bits. Note that the communication cost scales up with $1/\varepsilon$ because in the high-privacy regimes, the noise variance needs to be increased accordingly to provide stronger DP. Thus SecAgg's group size needs to be enlarged to capture the larger signal range and avoid catastrophic modular clipping errors. A similar phenomenon occurs for other additive noise-based mechanisms, e.g, the Skellam and binomial \cite{agarwal2018cpsgd, agarwal2021skellam} mechanisms.

However, we show that the $\Theta\lp d \log\lp d/\varepsilon^2 \rp \rp$ cost is strictly sub-optimal. In particular, the linear dependency on $d$ can be further improved when $n^2\varepsilon^2 \ll d$. To demonstrate this, we start by the following example to show that under a $(\varepsilon, \delta)$ central DP constraint, one can reduce the dimensionality to $m = O(n^2\varepsilon^2)$ without harming the MSE.

\paragraph{Dimensionality reduction under central DP} Consider the following simple project-and-perturb mechanism:

\begin{enumerate}
    \item The server generates a random projection matrix $S\in \mbb{R}^{m\times d}$ according to the sparse random projection defined in Section~\ref{sec:sparse_random_projection} and broadcasts it to $n$ clients.
    \item Each client sends $ y_i \eqDef \msf{clip}_{\ell_2, 1.1c}\lp S x_i \rp$.
    \item The server computes $\hat{\mu} \eqDef S^\intercal\lp \frac{1}{n}\sum_i y_i+N\lp 0, \sigma^2\mbb{I}_m \rp\rp$,  where $\sigma^2 = \Theta\lp \frac{c^2}{n^2\varepsilon^2}\rp$.
\end{enumerate}


We claim that the above project-and-perturb approach satisfies $(\varepsilon, \delta)$ DP and achieves the optimal MSE order. In other words, we can reduce the dimensionality \emph{for free}. 

To see why this is true, observe that we can decompose the overall $\ell_2$ error $\lV \hat{\mu} - \mu\rV^2_2$ into three parts: (1) the clipping error (i.e., $\lV y_i - Sx_i \rV^2_2$), (2) the compression error (i.e. $\lV\mu - S^\intercal S\lp\sum_i x_i/n\rp\rV^2_2$), and (3) the privatization error $\lV S^\intercal N(0, \sigma^2 \mbb{I}_m)\rV^2_2$. Then, we argue that all of them have orders less than or equal to $O\lp \frac{c^2d}{n^2\varepsilon^2} \rp$, as long as we select $m = \Theta(n^2\varepsilon^2)$ and $t = \Theta \lp \log d+ \log(n^2\varepsilon^2) \rp$.

First, the clipping error is small since the random projection $S$ satisfies the Johnson-Lindenstrauss (JL) property (see Lemma~\ref{lemma:SJL} in the appendix), which implies that $\lV S x_i\rV_2 \approx \lV x_i\rV_2 \leq c$ and that the clipping happens with exponentially small probability. Second, Lemma~\ref{lemma:proj_var_bdd} (in the appendix) suggests that compression error scales as $O\lp \frac{c^2d}{m} \rp$. Thus by picking $m = \Theta\lp n^2\varepsilon^2 \rp$, we ensure the compression error to be at most $O\lp \frac{c^2d}{n^2\varepsilon^2} \rp$. Finally, since the Gaussian noise $N$ added at Step 3 is independent of $S$, the privatization error can also be bounded by $O\lp \frac{c^2d}{n^2\varepsilon^2} \rp$.

We summarize this in the following lemma, where the formal proof is deferred to Section~\ref{proof:utility_cdp} in the appendix.

\begin{lemma}\label{lemma:utility_cdp}
Assume $\lV x_i \rV_2 \leq c$ for all $i \in [n]$. Then the output of the above mechanism $\hat{\mu}$ satisfies $\lp \varepsilon, \delta \rp$-DP. Moreover, if
$S$ (defined in \eqref{eq:def_S}) is generated with $m = \Theta(n^2\varepsilon^2)$ and $t = \Theta \lp \log d+ \log(n^2\varepsilon^2) \rp$, it holds that $\E\lb \lV \hat{\mu} - \mu \rV^2_2  \rb = O\lp\frac{c^2d }{n^2\varepsilon^2}\rp$.

\end{lemma}


\paragraph{Dimensionality reduction with SecAgg}
The above example shows that with a random projection, we can reduce the dimensionality from $d$ to $O(n^2\varepsilon^2)$ without increasing the MSE too much. Thus, under the distributed DP via SecAgg setting, we combine random projection with the DDG mechanism to arrive at our main scheme in Algorithm~\ref{alg:sketch_mean_decoder}. 

\begin{algorithm}[tb]
\caption{Private DME with random projection}\label{alg:sketch_mean_decoder}
\begin{algorithmic}
   \STATE {\bfseries Input:} Cleints' data $  x_1,...,x_n \in \mb{B}_{d}(c)$, compression parameter $m\in\mbb{N}$
   \STATE The server generates a sketching matrix $S \in \mbb{R}^{m\times d}$ \;
\STATE The server broadcasts $S$ to all clients\;
    
    \FOR{$i \in [n]$}
	\STATE Client $i$ computes $y_i \eqDef S x_i$ and $Z_i \eqDef \texttt{DDG}_{\msf{enc}}\lp y_i \rp \in \mbb{Z}_M^m$ with $\ell_2$ clipping parameter $1.1c$ (and other parameters being the same as in Algorithm~\ref{alg:ddg_simplified} with $d$ being replaced by $m$)\;
	\ENDFOR
    \STATE The server aggregates $Z_1,...,Z_n$ with SecAgg and decodes $\hat{\mu}_y = \frac{1}{n}\texttt{DDG}_{\msf{dec}}\lp\sum_{i\in[n]} Z_i\rp$\;
    \STATE The server computes $ \hat{\mu} = S^\intercal \hat{\mu}_y$.
    \STATE {\bfseries Return:} $\hat{\mu}$
\end{algorithmic}
\end{algorithm}

To control the $\ell_2$ error of Algorithm~\ref{alg:sketch_mean_decoder}, we adopt the same strategy as in Lemma~\ref{lemma:utility_cdp} (i.e., decompose the end-to-end error into three parts), with the privatization error being replaced by the error due to DDG. However, this will cause an additional challenge, as the error due to DDG is no longer independent of $S$ (as opposed to the Gaussian noise in the previous case). To overcome this difficulty, we leverage the fact that \emph{for any} projection matrix $S$, the (expected) $\ell_2$ error is bounded by $O\lp \frac{c^2m}{n^2\varepsilon^2} \rp$ and develop an upper bound on the final MSE accordingly (see Section~\ref{proof:random_projection_upper_bound} for a formal proof).

We summarize the performance guarantees of Algorithm~\ref{alg:sketch_mean_decoder} in the following theorem.
\begin{theorem}\label{thm:random_projection_upper_bound}
Let $S$ in Algorithm~\ref{alg:sketch_mean_decoder} be generated according to \eqref{eq:def_S} with $m = \Theta(n^2\varepsilon^2)$ and $t = \Theta \lp \log d+ \log(n^2\varepsilon^2) \rp$. Assume $\lV x_i \rV \leq c $ for all $i \in [n]$. Then as long as $n^2\varepsilon^2 \leq d$, the following holds:
\begin{itemize}
    \item Algorithm~\ref{alg:sketch_mean_decoder} satisfies $\lp \alpha, \frac{\varepsilon^2}{2}\alpha\rp$-RDP,
    \item the MSE is bounded by
    $ \E\lb \lV \hat{\mu} - \mu \rV^2_2 \rb = O\lp \frac{c^2d}{n^2\varepsilon^2} \rp, $
    \item the per-client communication is {\small
    $$ O\lp m\log\lp n+\sqrt{\frac{n^3\varepsilon^2}{m}}+\frac{\sqrt{m}}{\varepsilon} \rp\rp = O\lp n^2\varepsilon^2\log n \rp. $$}
\end{itemize}
\end{theorem}




\paragraph{Lower bounds for private DME with SecAgg}
Next, we complement our achievability result in Theorem~\ref{thm:random_projection_upper_bound} with a matching communication lower bound. Our lower bound indicates that Algorithm~\ref{alg:sketch_mean_decoder} is indeed optimal (in terms of communication efficiency), hence characterizing the fundamental privacy-communication-accuracy trade-offs. 

The lower bound leverages the fact that under \SA, the \emph{individual} communication budget each client has is equal to the \emph{total} number of bits the server can observe, which are all equal to the cardinality of the finite group $\mcal{Z}$ that \SA acts on. Therefore, even if each client sends a $b$-bit message (so the total information transmitted is $n\cdot b$ bits), the server still can only observe $b$ bits information. 

With this in mind, to give a per-client communication lower bound under \SA, it suffices to lower bound the total number of bits needed for reconstructing a $d$-dim vector (i.e. the mean vector $\mu$) within a given error (i.e. $O_\delta\lp c^2d/(n^2\varepsilon^2) \rp$). Towards this end, we first derive a general lower bound that characterizes the communication-accuracy trade-offs for compressing a \emph{single} $d$-dim vector in a centralized setting.

\begin{theorem}[compression lower bounds]\label{thm:compression_lb}
Let $v \in \mbb{R}^d$ and $\lV v \rV_2 \leq c$. Then for any (possibly randomized) compression operator $\mcal{C}: \mb{B}_{d}(c) \ra [2^b]$ that compresses $v$ into $b$ bits and any (possibly randomized) estimator $\hat{v}: [2^b] \ra \mb{B}_{d}(c)$, it holds that
\begin{equation}\label{eq:compression_lb_general}
    \min_{\lp \mcal{C}, \hat{v} \rp} \max_{v \in \mb{B}_d(c)} \E\lb \lV \hat{v}\lp \mcal{C}(v) \rp - v \rV^2_2 \rb \geq  c^22^{-2b/d}.
\end{equation}
Moreover, for any unbiased compression scheme (i.e., $\lp \mcal{C}, \hat{v} \rp$ satisfying $ \E\lb \hat{v}\lp \mcal{C}(v) \rp \rb = v$ for all $v \in \mb{B}_d(c)$) with $b < d$,  it holds that
\begin{equation}\label{eq:compression_lb_unbiased}
    \min_{\lp \mcal{C}, \hat{v} \rp} \max_{v \in \mb{B}_d(c)} \E\lb \lV \hat{v}\lp \mcal{C}(v) \rp - v \rV^2_2 \rb \geq  C_0c^2d/b,
\end{equation}
where $C_0 > 0$ is a universal constant.
\end{theorem}


Theorem~\ref{thm:compression_lb}, together with the fact that the per-client bit budget is also the total amount of information the server can observe, we arrive at the following lower bound.

\begin{corollary}
Consider the private DME task with SecAgg as described in Figure~\ref{fig1}. For any encoding function $\mcal{A}_{\msf{enc}}(\cdot)$ with output space $ \mcal{Z} $, if the $\ell_2$ estimation error $\E\lb \lV \hat{\mu} - \mu \rV^2_2 \rb \leq \xi$ for all possible $x_1,...,x_n \in \mb{B}_d(c)$, %
then it  must hold that
$ \log\lba  \mcal{Z}  \rba = \Omega\lp d\log\lp c^2/\xi \rp\rp. $
In addition, if $\hat{\mu}$ is unbiased and $\xi \leq c^2$, then
$ \log\lba  \mcal{Z}  \rba = \Omega\lp dc^2/\xi\rp. $
\end{corollary}



Finally, by plugging $\xi = O\lp \frac{c^2d}{n^2\varepsilon^2} \rp$ (which is the optimal $\ell_2$ error for the mean estimation task under centralized DP model), we conclude that 
\begin{itemize}
    \item $\Omega\lp \max\lp d\log\lp {n^2\varepsilon^2}/{d} \rp, 1\rp \rp$ bits of communication are necessary for general (possibly biased) schemes
    
    \item $\Omega\lp \min\lp n^2\varepsilon^2, d\rp \rp$ bits of communication are necessary for unbiased schemes.
\end{itemize}

We remark that the above lower bounds are both tight but in different regimes. Specifically, the first lower bound, which measures the accuracy in MSE, is tight for small $d$ but is meaningless in high-dimensional or high-privacy regimes where $d\gg n^2\varepsilon^2$. This also implies that $\tilde{\Omega}(d)$ bits are necessary for $d\ll n^2\varepsilon^2$ and that there is no room for improvement on DDG in this regime. On the other hand, the second bound is useful when $d = \Omega\lp n^2\varepsilon^2 \rp$ (with an additional unbiasedness assumption). This is a more practical regime for FL with SecAgg, and our scheme outperforms DDG in this scenario. %

\begin{remark}\label{rmk:unbiasedness}
Notice that in this work, we are mostly interested in unbiased estimators due to the following two reasons: 1) it largely facilities the convergence analysis of the SGD based methods, as these types of stochastic first-order methods usually assume access to an unbiased gradient estimator in each round. 2) In the high-dimensional or high-privacy regimes where $d\gg n^2\varepsilon^2$, the MSE is not the right performance measure since an estimator can have a large bias while still achieving a relative small MSE. 
For instance, in the regime where $n^2\varepsilon^2 \leq d$, the Gaussian mechanism has MSE $\Theta\lp \frac{c^2d}{n^2\varepsilon^2} \rp$; on the other hand, the trivial estimator $\hat{\mu} = 0$ achieves a smaller MSE, equal to $c^2 \leq O\lp\frac{c^2d}{n^2\varepsilon^2}\rp$, but such estimator gives no meaningful information. In order to rule out these impractical schemes, we hence impose the unbiasedness constraint.
\end{remark}




==> The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning (arxiv)_arXiv/content/6sparse.tex <==
Theorem~\ref{thm:random_projection_upper_bound} in Section~\ref{sec:worstcase} specifies the optimal trade-offs of private DME \emph{for all} possible datasets $x^n$. In other words, it provides a \emph{worst-case} (over all possible $x_i$) bound on the utility and shows that Algorithm~\ref{alg:sketch_mean_decoder} is worst-case optimal. However, we show in this section that with additional assumptions on the data, it is possible to improve the trade-offs beyond what is given in Theorem~\ref{thm:random_projection_upper_bound}. 

One such assumption is \emph{sparsity} of the data, which is justified by several empirical results that gradients tend to be (or are close to being) sparse. We hence study the sparse DME problem, which is formulated as in Section~\ref{sec:formulation} but with an additional $s$-sparsity assumption on $\mu$, i.e., $\lV \mu\rV_0 \leq s$. We present a sparse DME algorithm adapted from Algorithm~\ref{alg:sketch_mean_decoder}, showing that by leveraging the sparse structure of data, one can surpass the lower bound in Theorem~\ref{thm:random_projection_upper_bound}. Moreover, the dependency of communication cost and MSE on the model size $d$ becomes logarithmic.


\paragraph{DME via compressed sensing}
We adopt the same strategy as in Section~\ref{sec:worstcase}, (i.e., use a linear compression scheme to reduce dimensionality). However, instead of applying the linear decoder $S^\intercal\hat{\mu}_y$, we perform a more complicated compressed sensing decoding procedure and solve a (regularized) linear inverse problem. Specifically, we modify Algorithm~\ref{alg:sketch_mean_decoder} in the following way:
\begin{enumerate}
    \item For local compression, we replace the sparse random projection matrix $S\in \mbb{R}^{m\times d}$ with an $s$-RIP\footnote{See Definition~\ref{def:soft_re} for a weaker definition.} matrix (in particular, we use a Gaussian ensemble, i.e., $S_{i,j} \diid N(0, 1)$) and set $m = O\lp s\log d \rp$.
    \item To decode $\hat{\mu}$,  the server solves the following $\ell_1$ regularized linear inverse problem \eqref{eq:lasso} (i.e., LASSO \citep{tibshirani1996regression})
    where the $\lambda_n$ is set to be of the order $O\lp \frac{c\log d}{n\varepsilon}\rp$.
\end{enumerate}
With the above modifications, we arrive at Algorithm~\ref{alg:sparse_DME_lasso}:
\begin{algorithm}[ht]
    \begin{algorithmic}
	\STATE \textbf{Inputs:} clients' data $x_1,...,x_n$, sparse parameter $s$
	
	\STATE The server generates an compression matrix $S \in \mbb{R}^{m\times d}$ with $m = \Theta\lp s\log d \rp$ and $S_{i,j}\diid N(0, 1) $ and computes its largest singular value $\sigma_\msf{max}(S)$\;
	\STATE The server broadcasts $S, \sigma_\msf{max}(S)$ to all clients\;
	\FOR{$i \in [n]$}
	\STATE Client $i$ computes $y_i \eqDef S x_i$ and $z_i \eqDef \texttt{DDG}_{\msf{enc}}\lp y_i \rp \in \mbb{Z}_M^m$ with clipping rate $c' = c\sigma_\msf{max}(S)$ and dimension $d' = m$\;
	\ENDFOR
	
    \STATE The server aggregates $Z_1,...,Z_n$ with SecAgg and decodes $\hat{\mu}_y = \frac{1}{n}\texttt{DDG}_{\msf{dec}}\lp\sum_{i\in[n]} Z_i\rp$\;
    \STATE The server solves the following Lasso:
    \begin{equation}\label{eq:lasso}
        \hat{\mu} \in \arg\min_{x \in \mbb{R}^d}\lbp \frac{1}{m}\lV \hat{\mu}_y-Sx \rV_2+\lambda_n\lV x \rV_1 \rbp, 
    \end{equation} 
    where the regularization is picked to satisfy 
    $\lambda_n = O\lp \frac{c\log d}{n\varepsilon}\rp.$
	\STATE \textbf{Return: }{$\hat{\mu}$}
	\end{algorithmic}
	\caption{sparse DME via Compressed Sensing}\label{alg:sparse_DME_lasso}
\end{algorithm}

The next theorem provides the privacy and utility guarantees of Algorithm~\ref{alg:sparse_DME_lasso}.
\begin{theorem}[Sparse private DME]\label{thm:compressed_sensing_ddp}
Algorithm~\ref{alg:sparse_DME_lasso} satisfies $(\alpha, \frac{1}{2}\varepsilon^2\alpha)$-RDP. In addition, if $\lV \mu\rV_0 \leq s$, it holds that
\begin{itemize}
    \item the per-client communication cost is $O\lp s\log d \log \lp n^2 +{s\log d}/{\varepsilon^2}\rp\rp$;
    \item the MSE is bounded by $ O\lp \frac{c^2s\log^2 d}{n^2\varepsilon^2} \rp$.
\end{itemize}
\end{theorem}


Observe that under sparsity, both the accuracy and the communication cost depend on $d$ logarithmically. This implies that by leveraging the sparsity, we can replace $d$ with an ``effective'' dimension of $s\log d$. However, Algorithm~\ref{alg:sparse_DME_lasso} is more complicated than Algorithm~\ref{alg:sketch_mean_decoder} as it requires tuning hyper-parameters such as $s$ and $\lambda_n$.

\begin{remark}
The communication cost in Theorem~\ref{thm:compressed_sensing_ddp} no longer depends only on $n\varepsilon$, thus exhibiting a different behavior from the non-sparse case (i.e., that of  Theorem~\ref{thm:random_projection_upper_bound}). We remark that this is because we only present the result for the $s\log d \ll n^2\varepsilon^2$ (which is more reasonable in practice). However, one can extend the similar analysis in Section~\ref{sec:worstcase} and obtain the results for $s\log d \gg n^2\varepsilon^2$ regime.
\end{remark}








==> The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning (arxiv)_arXiv/content/7empirical.tex <==
We run experiments on the full Federated EMNIST and Stack Overflow datasets~\citep{caldas2018leaf}, two common benchmarks for \FL tasks. F-EMNIST has $62$ classes and $N=3400$ clients with a total of $671,585$ training samples. Inputs are single-channel $(28,28)$ images. The Stack Overflow (SO) dataset is a large-scale text dataset based on responses to questions asked on the site Stack Overflow. The are over $10^8$ data samples unevenly distributed across $N=342477$ clients. We focus on the next word prediction (NWP) task: given a sequence of words, predict the next words in the sequence. On both datasets, we select $n\in[100,1000]$ and $R=1500$. On F-EMNIST, we experiment with a $\approx 10^6$ parameter (4 layer) Convolutional Neural Network  (CNN) used by~\citet{kairouz2021distributed}. On SONWP, we experiment with a $\approx 4\cdot10^6$ parameter (4 layer) long-short term memory (LSTM) model---the same as prior work~\cite{andrew2019differentially,kairouz2021distributed}.
In both cases, clients train for $1$ local epoch using SGD. Only the server uses momentum.
For \DDP, we use the geometric adaptive clipping of~\cite{andrew2019differentially}.
We use the same procedure as~\citet{kairouz2021distributed}. We randomly rotate vectors using the Discrete Fourier Transform. We use their hyperparameter values for conditional randomized rounding and modular clipping. We communicate $16$ bits per parameter for F-EMNIST and $18$ for SONWP unless otherwise indicated.
We repeat all experiments with $5$ different seeds (or more, where stated).
We provide full detail on the models, datasets, and training setups in Appendix~\ref{app:models}, as well as the chosen values of the noise multiplier and sparse random projections (via sketching) parameters in Appendix~\ref{app:DP}. We provide details of our algorithms for sparse random projections (via sketching) in Appendix~\ref{app:sketching-practice}.

\begin{figure}[t!]
    \centering
    \captionsetup[subfigure]{width=0.95\linewidth}
    \begin{subfigure}[t]{0.48\linewidth}
        \includegraphics[width=0.97\linewidth]{figures/sonwp_1000.0_nm.pdf}
        \caption{\textbf{At $\mathbf{z\geq0.5}$, we attain $r\geq\mathbf{10}$x on SONWP} and without DP ($z=0$), $\approx4$x. $\Delta=4\%$. }
        \label{fig:sonwp}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/emnist_100.0_cr.pdf}
        \caption{\textbf{At $\mathbf{z\geq0.5}$ we attain $r\geq\mathbf{50}$x on F-EMNSIT}. Without DP, we cannot significantly compress. $\Delta=1\%$.}
        \label{fig:femnist}
    \end{subfigure}
    \caption{\textbf{Higher privacy requirements lead to higher attained compression rates with a slack of $\Delta$.} A higher (fixed) compression rate can also attain tighter privacy at no cost in performance.}
    
    \label{fig:puc}
\end{figure}


\paragraph{Analyzing the \puc tradeoff}\label{ssec:more-privacy-compression}
We now study the best compression rates that we can attain without significantly impacting the current performance.
For this, we train models that achieve state-of-the-art performance on the FL tasks we consider, and allow a slack of $\Delta=4\%$ relative to these models when trained without compression ($r=1$x). We first consider $z=0$, i.e., no DP, and see that about $r=4$x compression can be attained. However, recall that our theoretical results suggest that as $z$ increases and thus $\varepsilon$ decreases, fewer bits of communication are needed. Our experiments echo this finding: at $z=0.3$, we observe $r=5$x is now attainable and at $z\geq0.5$, $r=10$x is attainable. The highest $z$ we display can correspond both to a tighter privacy regime ($\varepsilon \approx 10$ or less) but, importantly also to models that are still highly performant indicating that a practitioner could reasonably select both these $z$ and $r$ to train models comparable to the state-of-the-art.
Our experiments on F-EMNIST in Figure~\ref{fig:femnist} show similar findings where fixing $r\geq50$x can attain $z\geq0.5$ for `free'. 
Finally, these results also corroborate that our bound of $\tilde{O}\lp \min(n^2\varepsilon^2, d) \rp$ is significantly less ($\approx 10$x) than that of~\citet{kairouz2021distributed} in practice.

Finding that we can significantly compress our models, another question that can be asked is `could a smaller model have been used instead?' To investigate this, we train a smaller model (denoted `small') which has only $\approx 2 \cdot 10^5$ parameters, which is comparable in size to the original CNN model updates compressed by $r\approx 5$x. We observe that this model has significantly lower performance ($>5pp$) across all privacy budgets when we compare them for a fixed latent dimension of $length \times width$. When we compress our original model beyond $r=5$x (smaller than the `small' model), we find that it still significantly outperforms it. These results indicate that training larger models do in fact attain higher performance even for the same latent update size: further, our results indicate we can enable training these larger models under the same fixed total communication.


\paragraph{Quantization or dimensionality reduction?}
Though we achieve significant compression rates from our linear dimensionality reduction technique, we now explore how these results compare with compression via quantization. Theoretically our bound can achieve a minimum compression independent of the ambient gradient size $d$. Because of this, we also expect our methods to outperform those based on quantization because their communication scales with $d$.

Our results in Figure~\ref{fig:quant-vary} and Table~\ref{tab:sonwp-b-vary} corroborate this hypothesis. We compare our compression against conditional randomized rounding to an integer grid of field size $2^b$. We vary the quantization (bits) per parameter $b$ while allowing the same $\Delta$ as above. Combined with dimensionality reduction, this gives a total communication per ambient parameter as $b/r$. When we use the vanilla distributed DP scheme of~\citet{kairouz2021distributed}, we find that we can only compress to $10$ bits per parameter on SONWP; if we instead favour our linear dimensionality reduction technique, we achieve a much lower $1.2$ bits per parameter (with $r=10$x and $b=12$). For F-EMNIST, we find we can compress down to $0.24$ bits per parameter at $z=0.5$ by optimizing both $b$ and $r$; this is much lower than using only quantization ($10$ bits per parameter) and a marginal increase over only dimensionality reduction ($0.27$). We observe $0.7$ bits per parameter at $z=0.3$ and $1.2$ at $z=0.1$. See Figure~\ref{fig:femnist-short} for results with $z=0.1,0.3$ and Figure~\ref{fig:femnist-long} for the comprehensive results at many $r$ and $b$, both in Appendix~\ref{app:figures}.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/emnist_0.5_shortnm.pdf}

    \caption{\textbf{Optimizing both $r$ and $b$ can further decrease communication}, to $0.24$ bits per parameter at $z=0.5$. See Figure~\ref{fig:femnist-short} of Appendix~\ref{app:figures} for $z=0.1,0.3$. Note that sometimes at higher bitwidths we observe lower performance within statistical error (standard deviation $\approx 1$)---here, we threshold to the highest accuracy of lower bitwidths to ease visualization. Full results without thresholding and all $r$ are in Figure~\ref{fig:femnist-long} of Appendix~\ref{app:figures}. These results used $30$ different seeds.}
    \label{fig:quant-vary}
\end{figure}
\begin{table}[h]
    \centering
    \begin{tabular}{c || c | c | c | c}
        \makecell{\small Noise\\ \small Multiplier, $z$ }& \makecell{\small Chosen Compression\\\small Rate $r$} & \makecell{\small Lowest Bit Width\\\small$b$ per Parameter} & \makecell{\small Total Communication\\\small Per Parameter} & \makecell{\small Final Test\\\small Performance, \%} \\
        \hline\hline
        \multirow{2}{*}{0.3} &
        1 & 10 & 10 & $21.90\pm 0.09$\\
        & \textbf{5} & \textbf{12} & \textbf{2.4} & $\mathbf{21.68\pm0.02}$\\
        \hline
        \multirow{3}{*}{0.5} &
        1 & 10 & 10 & $21.21 \pm 0.18$ \\
        & 5 & 12 & 2.4 & $21.11 \pm 0.08$ \\
        & \textbf{10} & \textbf{12} & \textbf{1.2} & $\mathbf{20.74 \pm 0.05}$ \\
        \hline
    \end{tabular}
    \caption{\textbf{Optimal compression can be found by tuning both the bit width $b$ and compression rate $r$.} Results for SONWP with 1000 clients. We find that increasing $r$ instead of $b$ achieves the highest total compression in all cases. Bold rows show the optimal compression parameters for the given $z$. We note that we cannot set lower than $b=10$ for this setting because SecAgg requires at least $O(\log{(n)}$ bits. The results in the final column take the form mean$\pm$standard deviation.}
    \label{tab:sonwp-b-vary}
\end{table}

Because of this, we now explore if raising the $b$ (decreasing quantization), past the max $b=18$ bits per parameter that we have considered thus far, will decrease the total communication. Inspecting $b=18\to22$ in Figure~\ref{fig:quant-vary} we do observe a marginal increase in test performance with increasing $b$ in some cases, indicating there may be potential to increase $r$. However, we do not find that we can significantly increase $r$ in these cases (see Figure~\ref{fig:femnist-long} of Appendix~\ref{app:figures}).


\paragraph{Impact of cohort size} 

We conduct experiments under (approximately, because varying $n$ impacts $\varepsilon$) fixed $\varepsilon$ to investigate how the cohort size $n$ impacts compression. From Theorem~\ref{thm:compression_lb}, we expect to see that as $n$ increases, so does does communication. Our empirical results closely match, shown in Figure~\ref{fig:n-sonwp} of Appendix~\ref{app:figures}. Further, we observe from Table~\ref{tab:n-emnist} of Appendix~\ref{app:figures} that under sufficiently high $z$, we can increase $n$ while keeping the total message size fixed (increase $r$ by $d/(\frac{n_2}{n_1}\frac{\log{n_2}}{\log{n_1}})$, where $n_2>n_1$) to \emph{improve the model performance}. In other words, in large $n$ scenarios where SecAgg can fail (due to large communication), our protocol may enable a practitioner to still increase $n$ to obtain better performance.


We attempted to improve compression rates by compressing layers separately (per-layer) or thresholding the noisy aggregate random projections. We found neither achieved significant improvements. The former aligns with results from~\citet{mcmahan2017learning} in central DP. See Appendix~\ref{app:ssec:per-layer-threshold} for this.



==> The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning (arxiv)_arXiv/content/8conclusion.tex <==
In this paper, we study the optimal privacy-communication-accuracy trade-offs under distributed DP via SecAgg. We show that existing schemes are order optimal when $d \ll n^2 \varepsilon^2$ and strictly sub-optimal otherwise. To address this issue, we provide an optimal scheme that leverages sparse random projections. We also show how our scheme can be minimally modified when the client updates are sparse to further improve the trade-offs. Our extensive experiments on FL benchmark datasets demonstrate significant communication gains ($\sim$10x) relative to existing schemes. Many important questions remain open, including obtaining a fundamental characterization of the privacy-accuracy-communication trade-offs under other models of distributed DP (e.g. via a trusted third-party or in a secure enclave as in \cite{bittau2017prochlo, GKMP20-icml, anon-power, ghazi2019private, ghazi2020pure, ishai2006cryptography, BalleBGN19, balle_merged, balcer2019separating, balcer2021connecting, girgis2020shuffled, girgis2021shuffled, erlingsson2019amplification}).  



==> The Fundamental Price of Secure Aggregation in Differentially Private Federated Learning (arxiv)_arXiv/macros.tex <==
\usepackage{xspace}
\usepackage{bbm}
\usepackage[shortlabels]{enumitem}
\usepackage{multirow}
\usepackage{makecell}




\newcommand{\FL}{FL\xspace}
\newcommand{\DP}{DP\xspace}
\newcommand{\ML}{ML\xspace}
\newcommand{\CNN}{CNN\xspace}

\newcommand{\DDP}{distributed DP\xspace}
\newcommand{\CEDP}{central DP\xspace}
\newcommand{\LDP}{local DP\xspace}
\newcommand{\SA}{SecAgg\xspace}
\newcommand{\puc}{privacy-utility-communication\xspace}
\newcommand{\PUC}{Privacy-Utility-Communication\xspace}

\newcommand{\SL}{\ensuremath{sketch\_length}\xspace}
\newcommand{\SW}{\ensuremath{sketch\_width}\xspace}


\usepackage{fixltx2e}
\usepackage{fancyvrb}
\RecustomVerbatimCommand{\VerbatimInput}{VerbatimInput}%
{fontsize=\footnotesize,
 framesep=2em, %
 rulecolor=\color{gray},
 commandchars=\|\(\), %
 commentchar=*        %
}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lb}{\left[}
\newcommand{\rb}{\right]}
\newcommand{\lbp}{\left\{}
\newcommand{\rbp}{\right\}}
\newcommand{\lba}{\left\lvert}
\newcommand{\rba}{\right\rvert}
\newcommand{\lV}{\left\lVert}
\newcommand{\rV}{\right\rVert}
\newcommand{\mv}{\middle\vert}
\newcommand{\ul}{\underline}
\newcommand{\ol}{\overline}
\newcommand{\mcal}{\mathcal}
\newcommand{\mscr}{\mathscr}
\newcommand{\what}{\widehat}
\newcommand{\wtild}{\widetilde}
\newcommand{\mb}{\mathbf}
\newcommand{\bbm}{\mathbbm}
\newcommand{\mbb}{\mathbb}
\newcommand{\msf}{\mathsf}
\newcommand{\la}{\leftarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\ua}{\uparrow}
\newcommand{\da}{\downarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\lgla}{\longleftarrow}
\newcommand{\lgra}{\longrightarrow}
\newcommand{\lglra}{\longleftrightarrow}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\llan}{\left\langle}
\newcommand{\rran}{\right\rangle}
\newcommand{\lce}{\left\lceil}
\newcommand{\rce}{\right\rceil}
\newcommand{\lfl}{\left\lfloor}
\newcommand{\rfl}{\right\rfloor}

\newcommand{\emphb}{\textcolor{blue}}
\newcommand{\emphg}{\textcolor{Grass}}
\newcommand{\emphr}{\textcolor{red}}
\newcommand{\eqFunc}{\overset{\mathrm{f}}{=}}
\newcommand{\eqDef}{\triangleq}
\newcommand{\diid}{\overset{\text{i.i.d.}}{\sim}}

\newcommand{\etal}{{\it et al.}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathsf{Var}}
\newcommand{\Cov}{\mathsf{Cov}}
\newcommand{\Bias}{\mathsf{Bias}}
\newcommand{\MSE}{\mathsf{MSE}}
\newcommand{\MLE}{\mathsf{MLE}}
\newcommand{\Risk}{\mathsf{R}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Ber}{\mathrm{Ber}}
\newcommand{\Poi}{\mathrm{Poi}}
\newcommand{\Binom}{\mathrm{Binom}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\SNR}{\mathsf{SNR}}
\newcommand{\INR}{\mathsf{INR}}
\newcommand{\SINR}{\mathsf{SINR}}
\newcommand{\Pe}{\mathsf{P}_{\mathsf{e}}}
\newcommand{\uPe}{\mathsf{\ol{P}}_{\mathsf{e}}}
\newcommand{\lPe}{\mathsf{\ul{P}}_{\mathsf{e}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\Indc}[1]{\mathbbm{1}_{\lbp #1\rbp}}
\newcommand{\Q}[1]{\mathrm{Q}\lp #1 \rp}
\newcommand{\FT}{\breve}
\newcommand{\ZT}{\check}
\newcommand{\sinc}{\mathrm{sinc}}
\newcommand{\rect}{\mathrm{rect}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}

